Benchmarking Complex Instruction-Following with Multiple Constraints Composition

Instruction following is one of the fundamental capabilities of large language models (LLMs). As the ability of LLMs is constantly improving, they have been increasingly applied to deal with complex human instructions in real-world scenarios. Therefore, how to evaluate the ability of complex instruction-following of LLMs has become a critical research problem. Existing benchmarks mainly focus on modeling different types of constraints in human instructions while neglecting the composition of different constraints, which is an indispensable constituent in complex instructions. To this end, we propose ComplexBench, a benchmark for comprehensively evaluating the ability of LLMs to follow complex instructions composed of multiple constraints. We propose a hierarchical taxonomy for complex instructions, including 4 constraint types, 19 constraint dimensions, and 4 composition types, and manually collect a high-quality dataset accordingly. To make the evaluation reliable, we augment LLM-based evaluators with rules to effectively verify whether generated texts can satisfy each constraint and composition. Furthermore, we obtain the final evaluation score based on the dependency structure determined by different composition types. ComplexBench identifies significant deficiencies in existing LLMs when dealing with complex instructions with multiple constraints composition.

==> tables/coherent_test.tex <==
% \begin{table*} [h]
% \centering
% \small
% \setlength{\tabcolsep}{1.6mm}{
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
% Nested Depth  & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c}{$ \geq $ 3}
% \\ 
% \midrule
% Setting & \textbf{OT} &  \textbf{CT}         & \textbf{OT}     & \textbf{CT} & \textbf{OT}     & \textbf{CT} \\
% \midrule
% \multicolumn{7}{c}{\textit{Closed-source Large Language Models}} \\
% \midrule
% GPT-4  & \textbf{0.725}  & \textbf{0.526}  &  \textbf{0.553}  & \textbf{0.340} & 0.446 & \textbf{0.216}  \\
% Claude-3-Opus  & 0.650  & 0.421    & 0.490  & 0.274  & \textbf{0.468} & 0.098   \\
% ChatGPT  & 0.513  &  0.158   & 0.376  & 0.179  & 0.273 & 0.020   \\

% \midrule
% \multicolumn{7}{c}{\textit{Open-source Large Language Models}} \\
% \midrule

% Qwen1.5-72B-Chat   & 0.650 & 0.368  & 0.506 & 0.255  & 0.388 & 0.078      \\
% Llama-3-70B-Chat  & 0.650  & 0.447  & 0.478  & 0.245 & 0.360 & 0.078   \\
% \midrule
% InternLM2-20B-Chat  & 0.563  &  0.316 & 0.380  &  0.142 & 0.331 & 0.020 \\
% Qwen1.5-14B-Chat  & 0.538  & 0.289  & 0.361 & 0.142  & 0.273 & 0.098 \\
% Baichuan2-13B-Chat   & 0.363  & 0.105  & 0.212 & 0.066 & 0.158 & 0.059 \\
% \midrule
% Llama-3-8B-Chat  & 0.475  & 0.237  & 0.294 & 0.075 & 0.230 & 0.020 \\
% Qwen1.5-7B-Chat  & 0.475  & 0.158  & 0.306 & 0.123 & 0.230 & 0.059 \\
% Mistral-7B-Instruct   & 0.463  & 0.237  & 0.282 & 0.094 & 0.245 & 0.039 \\
% InternLM2-7B-Chat  & 0.438  & 0.158  & 0.247 & 0.066 & 0.245 & 0.020 \\
% ChatGLM3-6B-Chat  & 0.275  & 0.053  & 0.145 & 0.019 & 0.108 & 0.000 \\

% \bottomrule
% \end{tabular}}
% \caption{The Coherent Test for Select Logic Compositionality}
% \label{tab:coherent_test}
% \end{table*}


\begin{table*} [h]
\centering
\small
\setlength{\tabcolsep}{1.6mm}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
Nesting Depth for \textbf{Selection}  & \multicolumn{3}{c|}{1} & \multicolumn{3}{c}{ $ \geq $ 2}
\\ 
\midrule
Setting & \textbf{OT} &  \textbf{CT}  & \textit{Relative $ \downarrow $}     & \textbf{OT}     & \textbf{CT} & \textit{Relative $ \downarrow $} \\
\midrule
\multicolumn{7}{c}{\textit{Closed-source Large Language Models}} \\
\midrule
GPT-4-1106  & 0.532  & 0.293  & 44.91\% & 0.491  & 0.146  & 70.29\% \\
Claude-3-Opus  & 0.498  & 0.293 &  41.21\% & 0.393  & 0.042  & 89.39\%  \\
GLM-4  & 0.546  & 0.307 &  43.79\% & 0.411  & 0.042  & 89.86\%  \\
GPT-3.5-Turbo-1106  & 0.338  &  0.093  & 72.55\%  & 0.166  & 0.018  & 92.07\%  \\

\midrule
\multicolumn{7}{c}{\textit{Open-source Large Language Models}} \\
\midrule

Qwen1.5-72B-Chat   & 0.461 & 0.271 & 41.11\% & 0.288 & 0.063 & 78.32\%  \\
Llama-3-70B-Chat  & 0.428  & 0.207 & 51.55\% & 0.313  & 0.042 & 86.68\% \\
\midrule
InternLM2-20B-Chat  & 0.338  &  0.121 & 64.11\% & 0.221  &  0.000 & 100.00\% \\
Qwen1.5-14B-Chat  & 0.305  & 0.121  & 60.17\% & 0.196 & 0.000 & 100.00\% \\
Baichuan2-13B-Chat   & 0.190  & 0.057 & 69.86\% & 0.110 & 0.000 & 100.00\% \\
\midrule
Llama-3-8B-Chat  & 0.234  & 0.057  & 75.60\% & 0.153 & 0.000 & 100.00\% \\
Mistral-7B-Instruct   & 0.201  & 0.043 & 78.65\% & 0.129 & 0.000 & 100.00\% \\
Qwen1.5-7B-Chat   & 0.286  & 0.100 & 65.06\% & 0.128 & 0.000 & 100.00\% \\
InternLM2-7B-Chat  & 0.230  & 0.079  & 65.91\% & 0.153 & 0.000 & 100.00\% \\
ChatGLM3-6B-Chat  & 0.160  & 0.036  & 77.66\% & 0.110 & 0.000 & 100.00\% \\

\bottomrule
\end{tabular}}
\caption{The Coherent Test for \textbf{Select} Composition Rules}
\label{tab:coherent_test}
\vspace{-4mm}
\end{table*}

==> tables/comparisons_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{0.9}
\label{tab:comparisons}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule

\multirow{2}{*}{Benchmark}  & \multirow{2}{*}{Data Size}  & \multicolumn{2}{c}{Constraint} & \multicolumn{3}{c}{Compositionality}  & \multirow{2}{*}{Evaluation Methods}    \\

\cmidrule(lr){3-4} \cmidrule(lr){5-7}
  & & Taxonomy  & Soft Constraints & \textbf{And.} & \textbf{Chain.}  & \textbf{Select.} &   \\               
\midrule

WizardLM Testset~\cite{xu2023wizardlm}    & 218  & -  & \CheckmarkBold & \CheckmarkBold   & - & -  & LLM Judge   \\

CELLO~\cite{he2023can}      & 523  & 4 & -  & \CheckmarkBold   & - & -  & Rule   \\

FollowBench~\cite{jiang2023followbench} & 820  & 5  &   \CheckmarkBold  & \CheckmarkBold             & - & - & LLM Judge \\

IFEval~\cite{zhou2023instructionfollowing} & 541  & 9-25 & - & \CheckmarkBold & -  & - & Rule  \\

CoDI-Eval~\cite{chen2024benchmarking}  & 9,060    & 5  & \CheckmarkBold  & \CheckmarkBold & -  & -  &  Classifier + Rule   \\

InfoBench~\cite{qin2024infobench} & 500 & 5   & \CheckmarkBold  & \CheckmarkBold  & - & -  & LLM Judge  \\

CoI Testset~\cite{hayati2024chain}   & 1,068  & -   &  \CheckmarkBold & - & \CheckmarkBold  & -  & Rouge + Human Evaluation   \\

\midrule
\textbf{\dataset{} (ours)}   & \textbf{1,263} & \textbf{4-18} & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \textbf{LLM Judge + Rule} 
\\ 

\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Comparisons between \dataset{} and other benchmarks, illustrating the features of \dataset{} in terms of dataset size, constraint, compositionality and evaluation methods. }
\vspace{-6mm}
\end{table*}

==> tables/scoring_questions.tex <==
\begin{CJK}{UTF8}{gbsn}
\begin{table*} [t]
\centering
\setlength{\tabcolsep}{1.6mm}{
\footnotesize
\begin{tabularx}{\linewidth}{p{4.5cm} X}
\toprule
\textbf{Instruction} & \textbf{Scoring Questions} \\

\midrule

Please introduce the following painting. Firstly, describe the information contained in the painting, and then introduce it according to the conditions:

- If the work contains any animal, the description should be in English, focusing on the animals depicted;

- If there is no animals, the description should be in Chinese, starting with the year of creation, followed by the background of the work’s creation, and finally, a brief summary of the work’s impact.

\

Painting: "Mona Lisa"
& 
\textbf{1}. Does the model first describe the information contained in "Mona Lisa"? (Helpfulness)

\textbf{2}. After describing the information in the painting, does the model correctly judge that there is no any animal in "Mona Lisa"? (Selection Logic, \textbf{Chain Logic-depends on 1})

\textbf{3}. Does the model introduce "Mona Lisa" in Chinese? (Target language, \textbf{Selection Logic-depends on 2})

\textbf{4}. Does the model first introduce the year of creation of "Mona Lisa"? (Helpfulness, \textbf{Selection Logic-depends on 2})

\textbf{5}. Does the model correctly introduce that the year of creation of "Mona Lisa" is 1503? (Factuality, \textbf{Selection Logic-depends on 2})

\textbf{6}. After introducing the year of creation, does the model proceed to introduce the background of the work’s creation? (Helpfulness, Topic, \textbf{Chain Logic-depends on 4})

\textbf{7}. Does the background of the work’s creation provided by the model is in accordance with facts? (Factuality, \textbf{Chain Logic-depends on 4})

\textbf{8}. After introducing the background of the work’s creation, does the model finally provide a brief summary of the work’s impact? (Helpfulness, Topic, \textbf{Chain Logic-depends on 6})

\textbf{9}. Does the summary of the work’s impact provided by the model is in accordance with facts? (Factuality, \textbf{Chain Logic-depends on 6})
\\
\bottomrule
\end{tabularx}}
\caption{An example of scoring questions}
\vspace{-4mm}
\label{tab:scoring_questions}
\end{table*}
\end{CJK}

==> tables/scoring_questions_zh.tex <==
\begin{CJK}{UTF8}{gbsn}
\begin{table*} [!h]
\centering
\setlength{\tabcolsep}{1.6mm}{
\small
\begin{tabularx}{\linewidth}{p{6cm} X}
\toprule
\textbf{Instruction} & \textbf{Scoring Questions} \\

\midrule

请你介绍以下绘画作品，先描述画面中包含的信息，然后根据条件按如下要求进行介绍：

- 如果其作品中包含动物意象，则整段介绍用英文，重点介绍其中的动物；

- 如果没有，则整段介绍用中文，要求先写出作品创作年份，然后写出作品的创作背景，最后简要概括作品的影响。

\ 

作品：《蒙娜丽莎》
& 
\textbf{1}. 模型是否先描述了《蒙娜丽莎》画面中包含的信息？（帮助性）

\textbf{2}. 模型是否在描述了画面中包含的信息后，正确判断画面中没有动物意象？（选择逻辑组合，\textbf{链式逻辑组合-依赖于1}）

\textbf{3}. 模型是否用中文进行介绍？（目标语言，\textbf{选择逻辑组合-依赖于2}）

\textbf{4}. 模型是否先说明了作品的创作年份？（帮助性，\textbf{选择逻辑组合-依赖于2}）

\textbf{5}. 模型是否正确说明《蒙娜丽莎》的创作年份为1503年？（事实性，\textbf{选择逻辑组合-依赖于2}）

\textbf{6}. 模型是否在说明了作品的创作年份后，写出了作品的创作背景？（帮助性，话题，\textbf{链式逻辑组合-依赖于4}）

\textbf{7}. 模型写出的作品创作背景是否符合事实？（事实性，\textbf{链式逻辑组合-依赖于4}）

\textbf{8}. 模型是否在写出了作品的创作背景后，最后简要概括了作品的影响？（帮助性，话题，\textbf{链式逻辑组合-依赖于6}）

\textbf{9}. 模型概括的作品影响是否符合事实？（事实性，\textbf{链式逻辑组合-依赖于6}）
\\

\midrule
Please introduce the following painting. Firstly, describe the information contained in the painting, and then introduce it according to the conditions:

- If the work contains any animal, the description should be in English, focusing on the animals depicted;

- If there is no animals, the description should be in Chinese, starting with the year of creation, followed by the background of the work’s creation, and finally, a brief summary of the work’s impact.

\

Painting: "Mona Lisa"
& 
\textbf{1}. Does the model first describe the information contained in "Mona Lisa"? (Helpfulness)

\textbf{2}. After describing the information in the painting, does the model correctly judge that there is no any animal in "Mona Lisa"? (Selection Logic, \textbf{Chain Logic-depends on 1})

\textbf{3}. Does the model introduce "Mona Lisa" in Chinese? (Target language, \textbf{Selection Logic-depends on 2})

\textbf{4}. Does the model first introduce the year of creation of "Mona Lisa"? (Helpfulness, \textbf{Selection Logic-depends on 2})

\textbf{5}. Does the model correctly introduce that the year of creation of "Mona Lisa" is 1503? (Factuality, \textbf{Selection Logic-depends on 2})

\textbf{6}. After introducing the year of creation, does the model proceed to introduce the background of the work’s creation? (Helpfulness, Topic, \textbf{Chain Logic-depends on 4})

\textbf{7}. Does the background of the work’s creation provided by the model is in accordance with facts? (Factuality, \textbf{Chain Logic-depends on 4})

\textbf{8}. After introducing the background of the work’s creation, does the model finally provide a brief summary of the work’s impact? (Helpfulness, Topic, \textbf{Chain Logic-depends on 6})

\textbf{9}. Does the summary of the work’s impact provided by the model is in accordance with facts? (Factuality, \textbf{Chain Logic-depends on 6})
\\
\bottomrule
\end{tabularx}}
\caption{An example of scoring questions}
\label{tab:scoring_questions_zh}
\end{table*}
\end{CJK}
